Body Part-Based Representation Learning for Occluded Person Re-Identification

Occluded person re-identification (ReID) is a person retrieval task which aims at matching occluded person images with holistic ones. For addressing occluded ReID, part-based methods have been shown beneficial as they offer fine-grained information and are well suited to represent partially visible human bodies. However, training a part-based model is a challenging task for two reasons. Firstly, individual body part appearance is not as discriminative as global appearance (two distinct IDs might have the same local appearance), this means standard ReID training objectives using identity labels are not adapted to local feature learning. Secondly, ReID datasets are not provided with human topographical annotations. In this work, we propose BPBreID, a body part-based ReID model for solving the above issues. We first design two modules for predicting body part attention maps and producing body part-based features of the ReID target. We then propose GiLt, a novel training scheme for learning part-based representations that is robust to occlusions and non-discriminative local appearance. Extensive experiments on popular holistic and occluded datasets show the effectiveness of our proposed method, which outperforms state-of-the-art methods by 0.7% mAP and 5.6% rank-1 accuracy on the challenging Occluded-Duke dataset. Our code is available at https://github.com/VlSomers/bpbreid.

==> sections/abstract_for_cmt.tex <==
Occluded person re-identification (ReID) is a person retrieval task which aims at matching occluded person images with holistic ones. For addressing occluded ReID, part-based methods have been shown beneficial as they offer fine-grained information and are well suited to represent partially visible human bodies. However, training a part-based model is a challenging task for two reasons. Firstly, individual body part appearance is not as discriminative as global appearance (two distinct IDs might have the same local appearance), this means standard ReID training objectives using identity labels are not adapted to local feature learning. Secondly, ReID datasets are not provided with human topographical annotations. In this work, we propose BPBreID, a body part-based ReID model for solving the above issues. We first design two modules for predicting body part attention maps and producing body part-based features of the ReID target. We then propose GiLt, a novel training scheme for learning part-based representations that is robust to occlusions and non-discriminative local appearance. Extensive experiments on widely used holistic and occluded datasets show the effectiveness of our proposed method, which outperforms state-of-the-art methods by 4.3% mAP and 6.1% rank-1 accuracy on the challenging Occluded-Duke dataset.






Occluded person re-identification (ReID) is a person retrieval task which aims at matching occluded person images with holistic ones. For addressing occluded ReID, part-based methods have been shown beneficial as they offer fine-grained information and are well suited to represent partially visible human bodies. However, training a part-based model is a challenging task for two reasons. Firstly, individual body part appearance is not as discriminative as global appearance (two distinct IDs might have the same local appearance), this means standard ReID training objectives using identity labels are not adapted to local feature learning. Secondly, ReID datasets are not provided with human topographical annotations. In this work, we propose BPBreID, a body part-based ReID model for solving the above issues. We first design two modules for predicting body part attention maps and producing body part-based features of the ReID target. We then propose GiLt, a novel training scheme for learning part-based representations that is robust to occlusions and non-discriminative local appearance. Extensive experiments on popular holistic and occluded datasets show the effectiveness of our proposed method, which outperforms state-of-the-art methods by 0.7% mAP and 5.6% rank-1 accuracy on the challenging Occluded-Duke dataset. Our code is available at https://github.com/VlSomers/bpbreid.

==> sections/acknowledgments.tex <==
\paragraph{Acknowledgment}
% \section*{ACKNOWLEDGMENT}
% UCLouvain + EPFL + Sport Radar | Synergy Sports
This work has been funded by Sportradar, by the Walloon region project ReconnAIssance, and by the Fonds de la RechercheScientifique – FNRS.


==> tables/components.tex <==
\begin{table}
\begin{center}
\caption{Ablation study for the main components of {\model} on Occluded-Duke.}
\label{table:components}
{\fontsize{8.5}{10}\selectfont{
\begin{tabular}{|l|cc|}
\hline%\noalign{\smallskip}
Methods & R-1 & mAP\\
%\noalign{\smallskip}
\hline
BoT \cite{BoT} baseline & 51.4 & 44.7 \\ % 3358
{\model} without learnable attention & 51.6 & 39.2 \\
{\model} without visibility scores & 52.6 & 45.3 \\ % 4349
{\model} without part-based triplet loss & 64.8 & 51.7 \\ % 4312
{\model} & \textbf{66.7} & \textbf{54.1} \\
\hline
\end{tabular}
}}
\end{center}
\end{table}

